CAMformer: Associative Memory is All You Need

Transformers face scalability challenges due to the quadratic cost of attention, which involves dense similarity computations between queries and keys. We propose CAMformer, a novel accelerator that reinterprets attention as an associative memory operation and computes attention scores using a voltage-domain Binary Attention Content Addressable Memory (BA-CAM). This enables constant-time similarity search through analog charge sharing, replacing digital arithmetic with physical similarity sensing. CAMformer integrates hierarchical two-stage top-k filtering, pipelined execution, and high-precision contextualization to achieve both algorithmic accuracy and architectural efficiency. Evaluated on BERT and Vision Transformer workloads, CAMformer achieves over 10x energy efficiency, up to 4x higher throughput, and 6-8x lower area compared to state-of-the-art accelerators--while maintaining near-lossless accuracy.

==> motivation/motivation.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{motivation/motivation.png}
    \caption{Attention as a key-lock mechanism. The query vector (Q) is used to determine similarity with stored keys (K), producing an attention score. The resulting soft selection determines which value vectors (V) to aggregate. This metaphor illustrates attention as an associative memory operation, where queries “unlock” relevant stored information.}
    \label{fig:key_lock_attention}
\end{figure}


\section{Background and Motivation}
\label{sec:background}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{circuit/main array.png}
    \caption{Array-level architecture of an example 2×6 BA-CAM module's array used for binary attention computation. Each row in the array performs parallel similarity matching against the broadcast query, with charge sharing accumulating match strength on shared matchlines. The inset shows the 10T1C CAM cell structure and an illustrative example of binary attention scoring based on Hamming similarity.}
    \label{fig:camformer-circuit}
\end{figure*}

\subsection{Limitations of Traditional Attention Mechanisms}
Transformer architectures have become foundational in various domains, including natural language processing, computer vision, and speech recognition, due to their ability to model long-range dependencies through self-attention mechanisms \cite{transformer_genomics, vision_transformer, transformer_complex_systems, transformer_machine_translation, transformer_retrosynthesis, transformer_NLP, transformer_biomedicine}. However, the computational and memory demands of these mechanisms, particularly the quadratic complexity associated with the QK$^\top$ and AV operations, pose significant challenges; these operations require extensive data movement and high computational resources, making them less efficient for long-sequence processing and deployment in resource-constrained environments \cite{transformer_complexity}. Traditional hardware accelerators often address this bottleneck by optimizing matrix multiplication operations inherent in the attention mechanism. Techniques like low-precision arithmetic, sparsity exploitation, and memory tiling have been employed to mitigate these challenges \cite{QUIDAM, EIE, SOFA}. Despite these efforts, the fundamental issue remains: the attention mechanism's reliance on dense matrix operations leads to substantial data movement and energy consumption.
\subsection{Content-Addressable Memory (CAM)} Content-Addressable Memory (CAM), also known as associative memory, is a specialized form of memory that enables data retrieval based on content rather than specific addresses \cite{cam_survey_1, cam_survey_2}. Unlike traditional Random Access Memory (RAM), where data is accessed by providing an explicit address, CAM allows for simultaneous comparison of input data against all stored entries, returning the address of matching data. This parallel search capability makes CAM exceptionally efficient for applications requiring rapid data matching and retrieval, such as IP look up, forwarding engine, Deep Random Forest acceleration, and DNA classification \cite{app_iplookup, app_forwarding_engine, app_DNA, app_DRF}. CAM operates by broadcasting the input data across the memory array, where each cell compares the input with its stored content. If a match is found, the corresponding address is returned. This mechanism eliminates the need for sequential searches, significantly reducing search time and enhancing performance in data-intensive tasks.
% Place the 2col float early so it can find a spot



\subsection{Aligning Attention with CAM Operations} 



The self-attention mechanism in Transformer architectures computes attention scores by comparing a query vector with a set of key vectors, followed by a weighted sum of corresponding value vectors \cite{AAUN}. Studies have shown that attention computation involves substantial matrix multiplications and data movement, leading to high computational and memory demands \cite{TRON, MatMul_is_significant, MatMul_is_significant2, MatMul_is_significant3}. By reinterpreting attention as an associative memory operation, we can leverage CAM's inherent parallelism to perform these computations more efficiently. In this paradigm, the query vector serves as the input to the CAM, which then retrieves the most similar key-value pairs based on predefined similarity metrics, such as Hamming distance or cosine similarity. This approach aligns with the fundamental operation of CAM, where data retrieval is based on content similarity. Implementing attention mechanisms using CAM can reduce computational overhead, minimize data movement, thereby enhancing scalability and energy efficiency.



% \begin{figure}[b]
%     \centering
%     \includegraphics[width=0.7\linewidth]{circuit/pvt.png}
%     \caption{I}
%     \label{fig:multiplication}
% \end{figure}


\subsection{Beyond Acceleration: Conceptual Alignment}
Most hardware accelerators for Transformer models focus on optimizing the computational aspects of attention mechanisms, often treating them as dense matrix operations to be approximated or compressed. 
These approaches prioritize performance gains while potentially overlooking the semantic essence of attention. 
In contrast, CAMformer adopts a fundamentally different approach by interpreting attention as an associative search process (see Fig. \ref{fig:key_lock_attention}). 
By implementing the semantics of attention directly in hardware through CAM structures, CAMformer not only accelerates attention computations but also preserves their conceptual integrity. 
This alignment between the computational model and hardware architecture yields significant benefits, including reduced energy consumption, and improved scalability. 
By transforming attention from a computational bottleneck into a native memory primitive, CAMformer paves the way for more efficient and semantically faithful implementations of attention mechanisms in hardware.



\begin{figure}[b]
    \begin{minipage}{0.5\textwidth}%
      \begin{subfigure}[t]{0.55\linewidth}
        \centering
        \includegraphics[width=\linewidth]{circuit/CapCAM_curves.png}
        \caption{}
        \label{subfig:circuit1}
      \end{subfigure}
      \begin{subfigure}[t]{0.44\linewidth}
        \centering
        \includegraphics[width=\linewidth]{circuit/pvt.png}
        \caption{} 
        \label{subfig:circuit2}
      \end{subfigure}
    \end{minipage}%
    \caption{(a) Matchline voltage traces for varying partial matches in 1×10 BA-CAM. (b) PVT analysis across corners for 16×64 array.}
\end{figure}

